The Expander Hierarchy and its Applications to Dynamic Graph Algorithms

We introduce a notion for hierarchical graph clustering which we call the expander hierarchy and show a fully dynamic algorithm for maintaining such a hierarchy on a graph with $n$ vertices undergoing edge insertions and deletions using $n^{o(1)}$ update time. An expander hierarchy is a tree representation of graphs that faithfully captures the cut-flow structure and consequently our dynamic algorithm almost immediately implies several results including: (1) The first fully dynamic algorithm with $n^{o(1)}$ worst-case update time that allows querying $n^{o(1)}$-approximate conductance, $s$-$t$ maximum flows, and $s$-$t$ minimum cuts for any given $(s,t)$ in $O(\log^{1/6} n)$ time. Our results are deterministic and extend to multi-commodity cuts and flows. The key idea behind these results is a fully dynamic algorithm for maintaining a tree flow sparsifier, a notion introduced by R\"acke [FOCS'02] for constructing competitive oblivious routing schemes. (2) A deterministic fully dynamic connectivity algorithm with $n^{o(1)}$ worst-case update time. This significantly simplifies the recent algorithm by Chuzhoy et al.~that uses the framework of Nanongkai et al. [FOCS'17]. (3) The first non-trivial deterministic fully dynamic treewidth decomposition algorithm on constant-degree graphs with $n^{o(1)}$ worst-case update time that maintains a treewidth decomposition of width $\text{tw}(G)\cdot n^{o(1)}$ where $\text{tw}(G)$ denotes the treewidth of the current graph. Our technique is based on a new stronger notion of the expander decomposition, called the boundary-linked expander decomposition. This decomposition is more robust against updates and better captures the clustering structure of graphs. Given that the expander decomposition has proved extremely useful in many fields, we expect that our new notion will find more future applications.

==> dynamic_ED_newer.tex <==

\newpage
\section{Fully Dynamic Expander Hierarchy}
\label{sec:dynamic_expander_decomposition}
%{\color{red}Things remains to do: (1) update $\alpha$ and $\phi$ accordingly; (2) add reference to theorems in previous sections; (3) tune some constants and other parameters;}

In this section, we will show an algorithm that maintains an expander hierarchy
of an unweighted simple graph that undergoes edge insertions and deletions. We
will always use $G$ to denote the current graph.
%The dynamic graph $G$ that we will be dealing with has $n$ vertices, and we let $m$ to be an upper bound of the number of edges in $G$ at any time, and we assume that $m=\poly(n)$ holds at any time. 
%For brevity, in this section we will refer to a \phied as a \emph{$\phi$-decomposition}, and refer to a \phiep as a \emph{$\phi$-partition}.
Our main result in this section is the following theorem:% and its corollary.
\begin{theorem}
\label{thm:dynamic_R_tree}
There is a randomized algorithm, that, given a fully dynamic unweighted graph
$G$ on $n$ vertices (undergoing adaptive edge insertions and deletions),
explicitly maintains, with high probability, a
$(2^{-O({\log^{1/2}n})},2^{-O(\log^{3/4}n)})$-expander hierarchy of $G$ in
amortized update time $2^{O(\log^{3/4} n)}$.
\end{theorem}
%\begin{corollary}
%There is a randomized algorithm that, given a fully dynamic graph $G$ on $n$ vertices (undergoing adaptive edge insertions and deletions), maintains, with high probability, a tree flow sparsifier for $G$ of quality $2^{-O(\log^{3/4}n)}$ in amortized update time $2^{O(\log^{3/4} n)}$.
%\end{corollary}

\iffalse
We first introduce the following definition that will be used
throughout the section. Given a pair of graphs $G_1=(V_1,E_1)$ and
$G_2=(V_2,E_2)$, we define the \emph{recourse} $\re(G_1,G_2)$ between $G_1$ and
$G_2$ to be the number of updates that is needed\thatchaphol{wrong definition}
to transform graph $G_1$ into $G_2$, where an update can be the insertion or
deletion of an edge, or the insertion or deletion of an isolated vertex.
Therefore, if the graphs $G_1$ and $G_2$ share a subgraph induced by
$V'\subseteq V_1\cap V_2$, namely $E_{G_1}(V')=E_{G_2}(V')$, then
$\re(G_1,G_2)\le|\Gamma_{G_1}(V')|+|E_{G_1}(V_1\setminus
V')|+|\Gamma_{G_2}(V')|+|E_{G_2}(V_2\setminus V')|$, since we can delete all
vertices of $V_1\setminus V'$ and all their incident edges in $G_1$, and then
insert all vertices of $V_2\setminus V'$ and their incident edges in $G_2$.
\fi

Fix $\phi=2^{-\Theta(\log^{3/4}n)}$, $\psi=2^{\Theta(\log^{1/2} n)}$,
$\alpha=1/\poly(\log n)$ and let $L=\log_{\psi}(n^2)=\Theta(\log ^{1/2}n)$. We
emphasize that these parameters are fixed throughout this section. (However, we
will use parameter $\alpha'$ and $\phi'$ as parameters that can depend on the
cluster $U$ we are referring to.)

We use the following lemma, whose proof is deferred to Section~\ref{apd:dynamic_expander_decomposition}.\thatchaphol{refer to the right sections.}
 
\begin{lemma}[Fully Dynamic Expander Decomposition]
\label{lem:fully_dynamic_expander_decomposition}
There is a randomized algorithm that, given any unweighted graph $G$ that
initially contains $m$ edges, undergoing a sequence of at most
$O(\phi\vol(G)/(38^{L}\cdot\psi/\alpha))$ adaptive insertions and deletions of
edges and isolated vertices, such that $|V(G)|\le n$ and $|E(G)|\le \poly(n)$
always holds,
%\thatchaphol{why do you need this? $n^{O(1)}$ ok?},
maintains an $(\alpha/38^{L},\phi/38^{L})$-expander decomposition in amortized update time $\tilde{O}(\psi\cdot 38^{2L}/(\alpha\phi^2))$ and pre-processing time $\tilde{O}(m/\phi)$. %Moreover, after $k$ updates, the number of new boundary edges is $O(k\psi)$.
Moreover, if we denote by $G'_t$ the contraction graph of $G$ after the $t^{th}$ update with respect to the decomposition maintained by the algorithm, then for each $k\ge 1$, $\sum_{t=1}^k\re(G'_t,G'_{t+1})\le O(k\cdot 38^{L}\cdot\psi/\alpha)$,
%\thatchaphol{From this statement, the ``recourse'' algorithm can update $G'_i$ to $G'_{i+1}$ in a much worse way that edit distance. You need to bound the ``recourse'', not the edit distance.}
%\thatchaphol{can handle any length of update sequence?}
where $\re(G_1,G_2)$ is the number of updates that  to transform graph $G_1$ into $G_2$.
\end{lemma}

We now complete the proof of Theorem~\ref{thm:dynamic_R_tree} using
Lemma~\ref{lem:fully_dynamic_expander_decomposition}. Throughout the proof, we
denote $\rho=38^{L}\cdot(\psi/\alpha)$, so $\rho=2^{\Theta(\log^{1/2} n)}$.


The algorithm proceeds in phases, and in each phase, we process the next
$f=\lfloor\phi m/\rho^{O(\log^{1/4} n)}\rfloor$ updates on $G$, where $m$ is
the volume of the current graph $G$ (that is, the graph at the end of the last
phase). Now we describe each phase in detail. We first preprocess the current
graph by computing an $(\alpha,\phi)$-EH $\tset$ of $G$ using the algorithm in
Theorem~\ref{thm:decomp}, as follows. We denote $G^0=G$, and we sequentially
compute, for each $i=0,1,2,\ldots,$ an $(\alpha,\phi)$-expander decomposition
of $G^i$, and then denote $G^{i+1}$ as the contraction graph of $G^{i}$ with
respect to the decomposition of $G^i$, until some graph $G^t$ contain no edges.
We denote by $\dep(\tset)$ the depth of $\tset$. Note that $\dep(\tset)$ may
change as $G$ undergoes updates. But since for each $0\le i\le \dep(\tset)-1$,
$\vol(G^{i+1})\le \tilde O(\phi)\cdot \vol(G^{i})$ always holds (from the
definition of an $(\alpha,\phi)$-expander decomposition), we know that
$\dep(\tset)\le O(\log^{1/4}n)$ holds throughout the algorithm.

We now show how to maintain $\tset$ within a phase. Upon an update on $G$, we
first update $G^0$ accordingly so that $G^0=G$ always holds, and then, for each
$0\le i\le \dep(\tset)-1$, we maintain an
$(\alpha/38^{L},\phi/38^{L})$-decomposition of $G^{i}$ using the algorithm of
Lemma~\ref{lem:fully_dynamic_expander_decomposition}, and maintain $G^{i+1}$ as
the contracted graph with respect to the partition. We now describe how to
maintain the $(\alpha,\phi)$-decomposition of the graphs
$G^0,G^1,\ldots,G^{\dep(\tset)-1}$. Upon an update on $G$, the graphs are
maintained sequentially in this order. The graph $G^0$ is maintained so that
$G^0=G$ always holds, and we also use the algorithm in Lemma
\ref{lem:fully_dynamic_expander_decomposition} to maintain an
$(\alpha/38^{L},\phi/38^{L})$-decomposition $\uset^0$ of $G^{0}$. Since
$f\le o(\phi m/\rho)$, the $(\alpha/38^{L},\phi/38^{L})$-decomposition
$\uset^0$ of $V(G^0)$ is valid throughout this
phase. %Put in other words, upon each update throughout this phase, we do not need to recompute $\uset^0$ from scratch.
The graph $G^1$ is then maintained as the contraction graph of $G^0$ with
respect to $\uset^0$. We now describe the maintenance of $G^i$, which amounts
to the maintenance of an $(\alpha/38^{L},\phi/38^{L})$-decomposition of graph
$G^{i-1}$. This is done in stages. In each stage, we apply the algorithm in
Lemma \ref{lem:fully_dynamic_expander_decomposition} to handle the next
$\lfloor\phi m'/\rho\rfloor$ updates on $G^i$, which is called the
\emph{length} of the stage, where $m'$ is the volume of the graph $G^i$ at the
beginning of the stage. Upon the current update on $G$, we assume that the
decompositions $\uset^0,\uset^1,\ldots,\uset^{i-2}$ are already maintained up
to this update.
%We distinguish between two cases, based on whether or not the decomposition $\uset^{i-2}$ of $V(G^{i-2})$ has been recomputed from scratch upon the current update. We first assume that this is not the case. 
We compare the new graph $G^{i-1}$ with the old one before the current update,
and denote by $\re$ the recourse between these two graphs. If $\re$ is less
than the length of the current stage, then we feed a sequence of $\re$ udpates
(the updates needed transform the old $G^{i-1}$ to the new $G^{i-1}$) to the
run of the algorithm of Lemma \ref{lem:fully_dynamic_expander_decomposition} in
the current stage. Note that this may force the current stage of $G^i$ to be
completed and start a new stage. If $\re$ is at least the length of the current
stage, then we terminate the current stage and start a new stage by recomputing
$\uset^{i-1}$ from scratch.
%We now consider the case where the decomposition $\uset^{i-2}$ of $V(G^{i-2})$ is recomputed from scratch. In this case we terminate the current stage of maintaining $\uset^{i-1}$ as well, and recompute $\uset^{i-1}$ from scratch based on the new $G^{i-1}$. Then we terminate the current stage and start a new stage by recomputing $\uset^{i-1}$ from scratch.
%Note that, from Lemma~\ref{lem:fully_dynamic_expander_decomposition}, one update in $G_0$ may cause amortized $O(\rho)^{i}$ updates in $G^{i}$. 
%\thatchaphol{Need much longer proof. This is seriously too sloppy. And I think it is wrong now. should be $\poly(\psi)^i$ or something like that.}
%Therefore, it is possible that, when an update in $G^0$ comes, the number of updates caused in $G^i$ is greater than $\phi \vol(G^i)/12$. 
%In this case, we simply terminate the current stage and recompute an $(\alpha,\phi)$-decomposition by from scratch  for $G^i$, using Theorem \ref{thm:strong_expander_decomposition}.
We then maintain $G^i$ as the contraction graph of $G^{i-1}$ with respect to
the decomposition $\uset^{i-1}$. This completes the description of maintaining
$\uset^{i-1}$ and $G^i$. From
Lemma~\ref{lem:fully_dynamic_expander_decomposition}, it is clear that at any
time in this phase, the $(\alpha/38^{L},\phi/38^{L})$-EH that we maintain is
valid.%\thatchaphol{need a proof.}

We now proceed to bound the amortized update time. Clearly, it takes $O(1)$ time to update $G^0$.
We first consider the amortized update time that is devoted to maintaining decomposition $\uset^0$ (and $G^1$).
At the beginning of each phase, from Theorem~\ref{thm:decomp} the time needed for recomputing the expander hierarchy is $\tilde O(m/\phi)$. We charge this uniformly to all updates handled in this phase (recall that there are a total of $f=\Omega(\phi m/\rho^{O(\log^{1/4}n)})$ of them), so each update is charged $\rho^{O(\log^{1/4} n)}/\phi^2=2^{O(\log^{3/4} n)}$.
On the other hand, from Lemma \ref{lem:fully_dynamic_expander_decomposition}, the amortized update time for maintaining the decomposition $\uset^0$ is $\tilde{O}(\psi\cdot 38^{2L}/(\alpha\phi^2))=2^{O(\log^{3/4} n)}$.
For each $1\le i\le \dep(\tset)$, the analysis for the amortized update time for maintaining $\uset^i$ and $G^{i+1}$ is similar to the analysis for $\uset^0$ and $G^{1}$. 
%Recall that we are guaranteed that, for each $1\le i\le \dep(\tset)$, $\vol(G^i)\le \tilde{O}(\phi/\alpha)\vol(G^{i-1})$. Therefore, $\vol(G^i)\le \tilde O(\phi/\alpha)^i\cdot m$.
Consider a stage for maintaining $\uset^i$, and let $m'$ be the volume of $G^i$ at the beginning of this stage.
We first assume for simplicity that we have not terminate the stage in the middle and recompute $\uset^i$ from scratch. 
Then at the beginning, the time for recomputing the decomposition $\uset^i$ is at most $\tilde O(m'/\phi)$. We charge this uniformly to the updates (on $G^{i}$) handled in this stage (recall that there are a total of $\Omega(\phi m')$ of them), so each update is charged $\tilde O(1/\phi^2)=2^{O(\log^{3/4} n)}$. From Lemma~\ref{lem:fully_dynamic_expander_decomposition}, the amortized update time (with respect to the updates on $G^i$) for maintaining $\uset^i$ is $\tilde{O}(\psi\cdot 38^{2L}/(\alpha\phi^2))=2^{O(\log^{3/4} n)}$. Therefore, the total amortized update time (with respect to the updates on $G^i$) within a stage is $2^{O(\log^{3/4} n)}$.
Note that, from Lemma~\ref{lem:fully_dynamic_expander_decomposition}, one update in $G^0$ may cause amortized $O(\rho)^{i}$ updates in $G^{i}$. 
Therefore, the amortized update time with respect to update on $G$ is $2^{O(\log^{3/4} n)}\cdot O(\rho)^{i}=2^{O(\log^{3/4} n)}$.
We now consider the case where a stage is terminated in the middle, and the decomposition $\uset^i$ is recomputed from scratch. Note that this is caused by large recourse between the graph $G^{i-1}$ before and after an update. We transfer the charge on the updates in the terminated stage to the amount of recourse (which is also the update needed on $G^i$), and since the recourse is larger than the length of the current stage, each unit of recourse is charged at most $O(1/\phi^2)=2^{O(\log^{3/4} n)}$. On the other hand, the time for recomputing $\uset^{i}$ is also uniformly charged to the amount of recourse, so each unit of recourse is again charged at most $2^{O(\log^{3/4} n)}$.
Therefore, from the charging scheme, and since one update in $G^0$ may cause $O(\rho)^{i}$ recourse in $G^i$, we conclude that the amortized update time for maintaining $\uset^i$ is $2^{O(\log^{3/4} n)}$.
%say that a new sub-phase is saturated if upon an update on $G$, the process for maintaining $G^i$ is forced to start an new phase and another one after it is completed. Recall that in this case we abort the current sub-phase and simply recompute an $(\alpha,\phi)$-decomposition.
%Therefore, if no new sub-phase is saturated, then one update in $G^0$ creates at most $O(\psi)^i$ updates in $G^i$, and the total update time is $\tilde O(\psi^{i}\cdot \psi \cdot6^{2L}/\alpha)=2^{O(\log^{3/4} n)}$ from Lemma~\ref{lem:fully_dynamic_expander_decomposition}.
%If a new phase is saturated (which means $\phi m'/12\le O(\psi)^i$), then recomputing its $(\alpha,\phi)$-decomposition takes time $O(\phi m'/\alpha)=O(\phi \cdot(\psi^{i}/\phi)/\alpha)=O(\psi^{i}/\alpha)$.
%Note that $O(\psi)^{\dep(\tset)}=2^{O(\log^{3/4} n)}$ always holds, so after $f$ updates to $G$, each graph in $\{G^i\}_{1\le i\le \dep(\tset)-1}$ may encounter at most $f\cdot O(\psi)^{\dep(\tset)}\le o(\phi m)$ updates in total.
Altogether, since $\dep(\tset)=O(\log^{1/4}n)$ throughout, we conclude that the amortized update time for maintaining the $(\alpha/38^L,\phi/38^L)$-EH is $2^{O(\log^{3/4} n)}$.

It remains to prove \Cref{lem:fully_dynamic_expander_decomposition}. We first describe useful subroutines that we need in \Cref{apd:dynamic_expander_decomposition} and then describe the algorithm for \Cref{lem:fully_dynamic_expander_decomposition} and prove its correctness in \Cref{sec:dyn decomp proof}.


==> dynamic_ED_sub1.tex <==
\subsection{\mlp and \cp}
\label{apd:dynamic_expander_decomposition}

In this section, we define a subroutine called \mlp, and then use it to construct another subroutine called \cp, which is further used to construct the algorithm of Lemma~\ref{lem:fully_dynamic_expander_decomposition}.

Below, whenever we work on some cluster $U$ that is $(\alpha',\phi')$-linked and we know both parameters $\alpha',\phi'$, we always set $w=\alpha'/\phi'$ when we call \Cref{thm:dynamic_expander_pruning}
as a subroutine. 



\subsubsection*{The Process \mlp}
Let $U$ be a cluster that is $(\alpha',\phi')$-linked in the graph $G$ in the beginning of the process for some parameters $0<\alpha',\phi'<1/2$ are known to us.\thatchaphol{$M_1$ can process sequence of updates instead of one batch}

The input to \mlp is the cluster $U$ and the parameters $\alpha',\phi'$. Upon up to $N=\lfloor\frac{\phi'\vol_{G}(U)}{1200}\rfloor$ updates on $G$ that are relevant to $U$ (i.e., the insertions and deletions of an edge whose at least one endpoint is in $U$), the process \mlp maintains a subset $P\subseteq U$ of vertices, such that the cluster $U\setminus P$ is $(\alpha'/38^L,\phi'/38^{L})$-linked in $G$.

The process \mlp will use the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} as a subroutine. We first introduce the some notations.
We denote by $D$ the sequence of updates on $G$ that are relevant to $U$. 
For a pair of integers $1\le i<j\le N$, we denote $D(i,j)$ as the subsequence of $D$ from the $i$th update to the $j$th update (including both). We call such a subsequence a \emph{batch}.  
For a cluster $W$ of vertices that is $(\alpha',\phi')$-linked in $G$ upon the $(i-1)$th update, we denote by $\mathcal{B}(W,i,j,\alpha',\phi')$ to be the run of the algorithm in Theorem~\ref{thm:dynamic_expander_pruning}, starting with the cluster $W$ in $G$ with boundary-linkedness parameters $\alpha'$ and $\phi'$, handling the updates in $D(i,j)$. Note that, an update on $G$ may be irrelevant of $W$ (i.e., both endpoints of the updated edge are not in $W$). In this case we simply ignore this update in the run of $\mathcal{B}(W,i,j,\alpha',\phi')$.

We now describe the process \mlp. The process utilizes $\tilde L=\lfloor\log_{\psi}N\rfloor$ machines that work in parallel.
Since $N\le |E(G)|\le n^2$, $\tilde L\le L=O(\sqrt{\log n})$.
We name the machines $M_1, \ldots, M_{\tilde L}$, respectively. Intuitively, the machines handle batches of updates of different sizes, and can also send messages to each other. For each $1\le s\le \tilde L$, we denote $R_s=\psi^s$, and let machine $M_s$ handle batches of size around $R_{s}$. The machine $M_1$ is the main machine, and it will maintain a pruned set $P^1$ upon each update, which is also the pruned set maintained by the \mlp{ }process.

We start by describing the work on machine $M_{\tilde L}$. It simply runs the algorithm of Theorem~\ref{thm:dynamic_expander_pruning} from the beginning to the end, with parameters $\alpha'$ and $\phi'$. Put in another way, machine $M_L$ runs $\mathcal{B}(U,1,N,\alpha',\phi')$. 
For each $1\le i\le N$, let $P^{\tL}_i$ be the set that it maintains after the $i$th update. 
The only machine that $M_{\tL}$ talks to is $M_{\tilde L-1}$. Specifically, for each $t\ge 1$, after the first $tR_{\tilde L-1}$ updates, $M_{\tL}$ sends the pruned set $P^L_{tR_{\tilde L-1}}$ to $M_{\tilde L-1}$. This completes the description of the work on machine $M_{\tL}$. %From Lemma~\ref{thm:dynamic_expander_pruning}, for each $i$, $\vol(P^L_i)=O(i/\phi)$, $|\Gamma_U(P_i)|=O(i)$, and the cluster $\overline{P^L_i}=U\setminus P^L_i$ is $(\alpha/38,\phi/38)$-linked in $G$.

We now describe the work on $M_s$ for each $2\le s\le \tilde L-1$. For each $1\le i\le N$, machine $M_s$ maintains a pruned set $P^{s}_{i}$, and for each $t\ge 1$, it sends the pruned set $P^{s}_{tR_{s-1}}$ to machine $M_{s-1}$.
For each $1\le t\le N/R_{s}$, the $t^{th}$ stage of $M_s$ deals with the batch $D((t-1)R_{s}+1, tR_{s})$ of updates, but with different parameters.
Specifically, in the first stage, $M_{s}$ runs $\mathcal{B}(U,1,R_{s},\alpha'/38^{\tilde L-s},\phi'/38^{\tilde L-s})$. For each $t>1$, at the beginning of the $t^{th}$ stage, $M_s$ receives the set $P^{s+1}_{(t-1)R_{s}}$ from machine $M_{s+1}$, and then it runs $\mathcal{B}(\overline{P^{s+1}_{(t-1)R_{s}}},(t-1)R_{s}+1,tR_{s},\alpha'/38^{\tilde L-s},\phi'/38^{\tilde L-s})$ throughout the stage, where $\overline{P^{s+1}_{(t-1)R_{s}}}=V\setminus P^{s+1}_{(t-1)R_{s}}$ and set the pruned set to be the union of (i) the pruned set maintained by $\mathcal{B}(\overline{P^{s+1}_{(t-1)R_{s}}},(t-1)R_{s}+1,tR_{s},\alpha'/38^{\tilde L-s},\phi'/38^{\tilde L-s})$; and (ii) the set $P^{s+1}_{(t-1)R_{s}}$.

\iffalse
See Figure~\ref{fig:life_of_machine} for an illustration.
\begin{figure}[h]
\centering
\subfigure[The work scheduling on of machine $M_s$.]
{\scalebox{.3}{\includegraphics{life_of_machine_s}}}
\hspace{0cm}
\subfigure[The nesting workzones of the machines.]
{\scalebox{.3}{\includegraphics{nesting_workzone}}}
\caption{An illustration of schedule on machines and their nested workzones.} \label{fig:life_of_machine}
\end{figure}
\fi

We now describe the work on machine $M_1$. The machine $M_1$ receives a message from $M_2$ after every $R_1=\psi$ updates, but do not send any messages to other machines.  The work on $M_1$ is also divided into stages, where in the $t^{th}$ stage, $M_1$ deals with the batch $D((t-1)R_{1}+1, tR_{1})$ of updates. 
In the first stage, for each $1\le t'\le R_1$, upon the $t'$th update, $M_{1}$ runs the entire $\mathcal{B}(U,1,t',\alpha'/38^{\tilde L-1},\phi'/38^{\tilde L-1})$ process before the next update comes. Put in other words, in the first stage, upon each update, the machine $M_1$ makes an individual run of the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} handling all updates (from the first update to the current update).
For each $t>1$, at the beginning of the $t^{th}$ stage, $M_1$ receives the set $P^2_{(t-1)R_1}$ from $M_2$, and then, for each $1\le t'\le R_1$, upon the $((t-1)R_1+t')$th update, $M_{1}$ runs the entire $\mathcal{B}(\overline{P^2_{(t-1)R_1}}, (t-1)R_1+1,(t-1)R_1+t',\alpha'/38^{\tilde L-1},\phi'/38^{\tilde L-1})$ process before the next update comes. This completes the description of the work on machine $M_1$. 

To summarize, the machines coordinate to work in a hierarchical way, in the sense that, the working graph of machine $M_s$ depends on the pruned sets of machines $M_{s+1}, \ldots, M_{\tilde L}$. When a machine with a larger index produces a pruned set, every machine with a smaller index works on the remaining graph where the pruned set is taken out from $U$.
%See Figure~\ref{fig:life_of_machine} for an illustration.

We prove the following claim on the boundary-linkedness of the pruned set.
\begin{claim}
\label{obs:cluster_linkedness}
For each $0\le s\le \tilde L-1$ and for each $t\ge 1$, for each cluster $P^{s+1}_{tR_s}$ that is produced by machine $M_{s+1}$, the cluster $\overline{P^{s+1}_{tR_s}}=U\setminus P^{s+1}_{tR_s}$ is $(\alpha'/38^{\tilde L-s}, \phi'/38^{\tilde L-s})$-linked in $G$.
\end{claim}
\begin{proof}
We prove by reverse induction on $s$. In the base case $s=\tilde L-1$, $M_{\tL}$ runs $\mathcal{B}(U,1,N,\alpha',\phi')$. 
Since $U$ is initially $(\alpha',\phi')$-linked in the graph $G$ when this \mlp{ }process is started, and $N\le \phi'\vol(U)/120$,
from Theorem~\ref{thm:dynamic_expander_pruning}, for each $t\ge 1$, the cluster $\overline{P^{\tilde L}_{tR_{\tilde L-1}}}$ is $(\alpha'/38, \phi'/38)$-linked in $G$. Assume that the observation is true for machines $M_{\tilde L-1},\ldots,M_{s+2}$. Consider now the machine $M_{s+1}$. In each stage, it simply runs the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} on cluster $\overline{P}$ in $G$ that  is $(\alpha'/38^{\tilde L-s-1}, \phi'/38^{\tilde L-s-1})$-linked in $G$, where $P$ is a set that $M_{s+1}$ received from $M_{s+2}$. 
We prove the following observations.
\begin{observation}
\label{obs:vol_decrease}
$\vol_G(\overline P)\ge \vol_G(U)/2^{\tL-s-1}$.
\end{observation}
\begin{proof}
From Theorem~\ref{thm:dynamic_expander_pruning},
$\vol_G(P^{\tL})\le \vol_{G[U]^w}(P^{\tL})\le \frac{32N}{\phi'}\le \frac{32}{\phi}\cdot \lfloor\frac{\phi'\vol_{G}(U)}{1200}\rfloor\le \frac{\vol_{G}(U)}{2}$.
Therefore, $\vol_{G}(\overline{P^{\tL}})\ge \frac{\vol_{G}(U)}{2}$. Similarly, for each $1\le s\le \tL$, $\vol_{G}(\overline{P^{s}})\ge \frac{\vol_{G}(U)}{2^{\tL-s-1}}$.
\end{proof}
From the above observation, we have
\[\psi^{s+1}\le \frac{N}{\psi^{\tL-s-1}} \le \frac{\phi'\vol_G(U)}{1200\cdot\psi^{\tL-s-1}}\le \frac{\frac{\phi'}{38^{\tL-s-1}}\cdot\vol_G(U)}{1200\cdot(\frac{\psi^{\tL-s-1}}{38^{\tL-s-1}})}
\le \frac{\frac{\phi'}{38^{\tL-s-1}}\cdot\vol_G(\overline P)}{1200\cdot(\frac{\psi^{\tL-s-1}}{38^{\tL-s-1}})}
\le \frac{\frac{\phi'}{38^{\tL-s-1}}\cdot\vol_G(\overline P)}{1200}.\]
Note that $\vol_G(\overline P)=  \vol(G[\overline P]^{1})\le \vol(G[\overline P]^{\alpha'/\phi'})$, the number of updates handled in a stage of $M_{s+1}$ is proper for the run of the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} within the stage.
From Theorem~\ref{thm:dynamic_expander_pruning}, the pruned set $P'$ maintained by $M_{s+1}$ will always satisfies that $\overline{P'}$ is $((1/38)\cdot\alpha'/38^{\tilde L-s-1}, (1/38)\cdot\phi'/38^{\tilde L-s-1})$=$(\alpha'/38^{\tilde L-s}, \phi'/38^{\tilde L-s})$-linked in $G$. 
%This completes the proof of this observation.
\end{proof}
%The following corollary follows easily from Theorem~\ref{thm:dynamic_expander_pruning} and Observation~\ref{obs:cluster_linkedness}.\thatchaphol{Please prove this. In particular, why $\psi$ appears in only one of the bound?}
\begin{corollary}
\label{cor:mlp_prune}
At any time, the cluster $U\setminus P^1$ maintained by the \mlp{ }process is $(\alpha'/38^L,\phi'/38^L)$-linked in $G$.
\end{corollary} 
\begin{proof}
From Claim \ref{obs:cluster_linkedness}, at any time, the cluster $U\setminus P^1$ is $(\alpha'/38^{\tL},\phi'/38^{\tL})$-linked in $G$.
Since $\tL\le L$, the cluster $U\setminus P^1$ is also $(\alpha'/38^{L},\phi'/38^{L})$-linked in $G$.
\end{proof}
\begin{corollary}
\label{cor:mlp_update_time}
For each $2\le s\le \tilde L$, the amortized update time for machine $M_s$ is $\tilde{O}((38^{L-s}/\phi')^2)$.
The amortized update time for machine $M_1$ is $\tilde{O}(\psi\cdot(38^{L}/\phi')^2)$.
\end{corollary} 
\begin{proof}
Fix an index $2\le s\le \tL$.
From Claim~\ref{obs:cluster_linkedness}, we know that, in each stage of $M_s$, the initial working cluster is $(\alpha'/38^{\tilde L-s}, \phi'/38^{\tilde L-s})$-linked in $G$.
From Theorem~\ref{thm:dynamic_expander_pruning}, the amortized update time by $M_s$ is $\tilde O((38^{\tilde L-s}/\phi')^2)=\tilde O((38^{L-s}/\phi')^2)$.
Consider now machine $M_1$, from Claim~\ref{obs:cluster_linkedness}, in each stage of $M_1$, the initial working cluster is $(\alpha'/38^{\tilde L-1}, \phi'/38^{\tilde L-1})$-linked in $G$. Recall that upon each update, the machine $M_1$ makes an individual run of the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} handling all updates in this stage so far (there are at most $\psi$ of them).
From Theorem~\ref{thm:dynamic_expander_pruning}, the amortized update time by $M_1$ is $\tilde O(\psi\cdot(38^{\tilde L}/\phi')^2)=\tilde O(\psi\cdot(38^{L}/\phi')^2)$.
\end{proof}




\iffalse
From this proposition, it is not hard to see that, after the first $t$ updates, the volume of the pruned set maintained by machine $M_i$ is 
$O(\sum_{j=0}^{i}t\cdot 38^{L-j}/\phi)=O(t\cdot 38^{L-i}/\phi)$. Therefore, after the first $t$ updates, the volume of the pruned set maintained by $M_1$ is $O(t\cdot 38^{L}/\phi)$.

From this proposition and Lemma~\ref{thm:dynamic_expander_pruning}, after each update, the number of new boundary edges created by $M_1$ is $O(\psi)$. For the machine $M_s$ where $2\le s\le L$, after each phase of $R_s$ updates, it creates $O(R_s)$ new boudaries. Therefore, the amortized number of new boundary edges created by $M_s$ is $O(1)$. We can therefore conclude that, after the first $t$ updates the total number of new boundary edges created by all machines is $O(t\psi)$.



The following observation follows easily from Theorem~\ref{thm:dynamic_expander_pruning}.
\begin{observation}
	$\vol_{G}(P)= O(i\cdot6^{L}/\phi)$.
\end{observation}\fi

==> dynamic_ED_sub2.tex <==

\iffalse
In this section we provide the proof of Lemma~\ref{lem:fully_dynamic_expander_decomposition}.
%Recall that $\phi=2^{-\Theta(\sqrt{\log m})}$, $\psi=2^{\Theta(\log^{3/4} m)}=n^{o(1)}$, and $L=\log_{\psi}m=\Theta(\log^{1/4}m)$.
We will use the following auxiliary lemma, which can be seen as a variant of Lemma~\ref{lem:dynamic_expander_pruning}, whose proof is deferred to
Section~\ref{sec:advanced_expander_pruning}.
\begin{lemma}
\label{lem:advanced_dynamic_expander_pruning}
There is a deterministic algorithm, that, given any graph $G=(V,E)$ on $n$ vertices that initially contains $m$ edges, a cluster $U$ that is $(\alpha,\phi)$-linked in the initial graph $G$, and a sequence of at most $\phi m/12$ updates on $G$, where an update can be an edge insertion or an edge deletion, maintains a pruned set $P\subseteq U$ of vertices such that the following property holds. For each $i\ge 1$, denote by $P_i$ ($G_i$, resp.) the set $P$ (graph $G$) after the $i$th update. We have, for all $i$,
\begin{enumerate}
\item $\vol_{G_0}(P_i)= O(i\cdot6^{L}/\phi)$; note however that $P_i\subseteq P_{i+1}$ does not necessarily hold;
\item the cluster $V\setminus P_i$ is $(\alpha/38^L,\phi/38^{L})$-linked in $G_i$; and
%\item the number of boundary edges of $U\setminus P$ over the first $i$ updates is at most $O(i\cdot\psi)$.
\item $\sum_{1\le t\le i}\dist(G_t[V\!\setminus\!P_t], G_{t+1}[V\!\setminus\!P_{t+1}])\le O(i\cdot\psi)$.
\end{enumerate}
Moreover, the amortized update time is $\tilde{O}(\psi\cdot(38^L/\phi)^2)$.
\end{lemma}
\fi

\subsubsection*{The Process \cp}
Before defining the process \cp, we need the following notations on the process \mlp.
Fix an index $1\le i\le N$. We define the set $\tilde P^{L}_{i}$ as the latest pruned set sent from $M_L$ to $M_{\tL-1}$ upon the $i$th update, namely 
$\tilde P^{\tL}_{i}=P^{\tL}_{R_{\tL-1}\cdot\lfloor i/R_{\tL-1}\rfloor}$.
For each $2\le s\le \tL-1$, we define $\tilde P^{s}_{i}=P^{s}_{R_{s-1}\cdot\lfloor i/R_{s-1}\rfloor}\setminus P^{s+1}_{R_{s}\cdot\lfloor i/R_{s}\rfloor}$.
Intuitively, the set $\tilde P^{s}_{i}$ is the latest progress made by machine $M_s$ in its current stage, that has been sent to machine $M_{s-1}$.
Lastly, we define the set $\tilde P^1_i=P^{1}_{i}\setminus P^{2}_{R_{1}\cdot\lfloor i/R_{1}\rfloor}$ as the pruned set maintained by the local prune process on machine $M_1$.
By definition, the sets $\tilde P^{1}_{i},\tilde P^{2}_{i},\ldots,\tilde P^{\tL}_{i}$ are mutually disjoint.
From the \mlp, it is easy to verify that, for each $1\le s\le \tL-1$, the working cluster for $M_s$ in its current stage is $U\setminus (\bigcup_{s+1\le j\le \tL}\tilde P^s_i)$, and $P^1_i=\bigcup_{1\le j\le \tL}\tilde P^s_i$.
We sometimes omit the subscript $i$ in the above definitions when the index $i$ refers to the index of the current update.

Similar to \mlp, let $U$ be a cluster that is $(\alpha,\phi')$-linked in the graph $G$ in the beginning of the process for some parameter $0<\phi'<1/2$ is known to us.
The input to \cp (CD-process) is the cluster $U$ and the parameter $\phi'$.
%\thatchaphol{Is this ok?}\thatchaphol{We do not need that $\phi' > \phi$ for the proof about \cp process, right? so I removed it}\thatchaphol{Emphasize again that the cluster $U$ that \cp works on is always w.r.t. original $\alpha$. }
%the input to \cp (CD-process) is a cluster $U$ that is $(\alpha,\phi')$-linked in the current graph $G$, for some parameter $\phi'\ge \phi$ that is known to us. 
We refer to $U$ as the \emph{working cluster} of the CD-process.
Upon up to $N=\lfloor\frac{\phi'\vol_{G}(U)}{1200}\rfloor$ updates
%\thatchaphol{should be $G[U]^w$ for some $w$?} 
on $G$ that are relevant to $U$, the CD-process maintains an $(\alpha/38^L,\phi'/38^{L})$-expander decomposition of $U$. 
%Namely, each cluster in this partition is $(\alpha/38^L,\phi/38^{L})$-linked in the current graph $G$.
In particular, the CD-process will use \mlp as a subroutine to maintain a set $P^1\subseteq U$, such that $U\setminus P^1$ is $(\alpha/38^L,\phi'/38^L)$-linked in $G$, and additionally, for each $1\le s\le \tL$, the CD-process will maintain a sub-partition of vertices in $\tilde P^s$. Clearly, these sub-partitions, together with the cluster $U\setminus P^1$ maintained by the \mlp process on $U$, form a partition of $U$, and this partition of $U$ is the decomposition maintained by the CD-process.  
%Moreover, from Theorem~\ref{thm:dynamic_expander_pruning}, for each $1\le s\le L$, $\vol_G(\tilde P^s)\le O(\psi^{s}\cdot 38^L/\phi)$.

We now describe the CD-process in detail. 
%Denote $m=\vol_{G}(U)$. 
The CD-process is defined recursively. When the number of vertices in its input cluster $U$ is below some large enough constant $c_0$, then upon each update, the CD-process simply recomputes the $(\alpha,\phi')$-expander decomposition on $U$ in $G$. 
%by computing the sparsity of each cut by brute force. 
Clearly, the update time is $O(1)$. 
Now we define the CD-process when the number of vertices in $U$ is larger than $c_0$.
%Assume now that the CD-process for all clusters of size at most $k$ are defined\thatchaphol{what is $k$? some constant?}, consider now the case where $U$ contains $k+1$ vertices. 
We start a \mlp process on $U$, maintaining the sets $\tilde P^1,\ldots,\tilde P^{\tL}$. Recall that, from \mlp, for each $1\le s\le \tL$, the set $\tilde P^s$ changes every $R_{s-1}$ updates, and as it changes, the sets $\tilde P^{s-1},\ldots,\tilde P^{1}$ becomes $\emptyset$. 
For each $1\le s\le \tL$, whenever the set $\tilde P^s$ changes, we compute an $(\alpha,\phi')$-decomposition on $\tilde P^{s}$ using the algorithm in Theorem~\ref{thm:decomp}. 
For each cluster $U'' \subseteq \tilde P^{s}$ from the decomposition for which \Cref{thm:decomp} also returns $\phi'' \ge \phi'$ and guarantees that $U$ is $(\alpha,\phi'')$-linked in $G$, we start a CD-process on it with $\alpha,\phi''$ as the parameters, that we also refer to as a \emph{sub-CD-process} of the CD-process on $U$.

The CD-process on the cluster $U$ is terminated whenever it has handled $N$ updates relevant to $U$. We say that a cluster $U$ \emph{expires} if the CD-process on it has just been terminated.
Whenever some cluster $U$ expires, we immediately terminate all its sub-CD-process, and then recompute an $(\alpha,\phi)$-expander decomposition on $U$ in the current graph and start a new CD-process on each cluster in the obtained decomposition. We call this step \emph{recycling}.  This finishes the description of the process \cp.
%Note that, since $\tilde P^1$ changes upon each update, we recompute an $(\alpha,\phi)$-decomposition on the new cluster $\tilde P^{1}$ upon each update as well.

We use the following observations on analyzing the update time of \cp.
%The following observations follow from the definition of sets $\{\tilde P^s\}_{1\le s\le \tL}$, the definition of an $(\alpha,\phi')$-decomposition, Theorem~\ref{thm:decomp} and Theorem~\ref{thm:dynamic_expander_pruning}, and the property of \mlp that a stage on machine $M_s$ has length $O(\psi^{s})$.
\begin{observation}
\label{obs:downward_inter}
For each $1\le s\le \tL$, at any time, $|E(\tilde P^s, V\setminus \tilde P^s)|\le O(\psi^s/\alpha)$.
\end{observation}
\begin{proof}
From Claim~\ref{obs:cluster_linkedness}, the working graph at the beginning of each stage on machine $M_s$ is $(\alpha/38^{\tL-s}, \phi'/38^{\tL-s})$-linked in $G$.
From the discussion in the proof of Claim~\ref{obs:cluster_linkedness}, the number of updates handled in a stage of $M_{s+1}$ is proper for the algorithm of the run of the algorithm in Theorem~\ref{thm:dynamic_expander_pruning} within the stage.
Therefore, from the second property of Theorem~\ref{thm:dynamic_expander_pruning}, the number of edge between $\tilde P^s$ and $U\setminus(\bigcup_{s\le j\le \tL}\tilde P^j))$ is at most $O(\psi^s)$. From the third property of Theorem~\ref{thm:dynamic_expander_pruning}, the number of edges between $\tilde P^s$ and $(V\setminus U)\cup (\bigcup_{s\le j\le \tL}\tilde P^j)$ is at most $O(\psi^s/\alpha)$. Altogether, we have $|E(\tilde P^s, V\setminus \tilde P^s)|\le O(\psi^s/\alpha)$.
\end{proof}
\begin{observation}
\label{obs:intra}
For each $1\le s\le \tL$, at any time, the number of inter-cluster edges between clusters of the CD-process on $U$ in $\tilde P^s$ is at most $\tilde O(\psi^s\cdot 38^{L})$.
\end{observation}
\begin{proof}
From the definition of \mlp and Theorem~\ref{thm:dynamic_expander_pruning}, the volume of $\tilde P^s$ is always at most $O(\psi^{s}/(\phi'/38^{\tL}))$. From the definition of an $(\alpha,\phi')$-expander decomposition, the number of inter-cluster edges between the cluster in $\tilde P^s$ is at most $\tilde O( \phi'\cdot\psi^{s}/(\phi'/38^{\tL}))=\tilde O(\psi^s\cdot 38^{L})$.
\end{proof}





\paragraph{Amortized update time of \cp.}
Since the CD-process is defined recursively, the CD-process on a cluster $U$
may have other CD-process running on sub-clusters of
$U$. %We call them sub-CD process. Therefore,
It is easy to see that, within a CD-process, all working-clusters of
sub-CD-process form a laminar family. For the CD-process on $U$, from
Observation~\ref{obs:vol_decrease} $\vol(U\setminus P^1)\ge
\vol(U)/2$. %\thatchaphol{We are working on $G[U]^w$, this volume is w.r.t. which graph?}
%\zihan{need to tune the parameters, including $N$ and the number of updates in Lemma~\ref{lem:fully_dynamic_expander_decomposition}}
Therefore, for each of its sub-CD-process, the volume of its working graph is at most $1/2$ the volume of $U$.


If an update is the insertion or deletion of an isolated vertex $u$, then all
sub-CD-process of $U$ whose working cluster contains $u$ forms a chain:
$u\in U_1\subseteq U_2\subseteq\ldots\subseteq U_r=U$. Moreover, for each
$1\le i\le r-1$, $\vol(U_{i+1})\le\vol(U_i)/2$. Therefore, the number of these
working clusters is at most $O(\log n)$, and the CD-process on $U$ takes
$O(\log n)$ time to handle it. Now consider an update that is the insertion or
deletion of an edge $(u,u')$. Similarly, all the sub-CD-process containing $u$
or $u'$ form two chains. Consider now the work in the CD-process on $U$ alone
(without taking into account the work of its sub-CD-process). For each
$1\le s\le \tL$, an $(\alpha,\phi')$-expander decomposition on $\tilde P^s$ is
recomputed after every $\psi^s$ updates on $\tilde P^s$. Therefore, from
Theorem~\ref{thm:decomp} and Observation~\ref{obs:downward_inter}, the
amortized update time for computing an $(\alpha,\phi')$-decomposition on
$\tilde P^{s}$ is
$$\tilde O\left(\frac{1}{\psi^s}\left(\frac{|E(\tilde P^s, V\setminus \tilde P^s)|}{\phi'^2}+\frac{\vol(\tilde P^s)}{\phi'}\right)\right)=\tilde O\left(\frac{1}{\psi^s}\left(\frac{\psi^s}{\alpha \phi'^2}+\frac{\psi^s/(\phi'/38^{\tL})}{\phi'}\right)\right)=\tilde O\left(\frac{38^{L}}{\alpha\phi'^2}\right)
,$$ as $\tL\le L$.
Therefore, the total amortized update time for computing the $(\alpha,\phi')$-decompositions on $\tilde P^{1},\ldots,\tilde P^{\tL}$ is $\tilde O\left(\frac{38^{L}}{\alpha\phi'^2}\right)$.
Together with Corollary~\ref{cor:mlp_update_time}, the CD-process on $U$ alone handles the update in $\tilde{O}(\frac{\psi\cdot16^{2L}}{\alpha\phi'^2})$ amortized time. It is easy to see that the amortized update time of each sub-CD-process in the chain is bounded by that of the CD-process on $U$. We claim that the CD-process on $U$ (together with all its sub-CD-process) takes $\tilde{O}(\frac{\psi\cdot16^{2L}}{\alpha\phi'^2})$ amortized time in handling an update.





%For a cluster $U\subseteq V(G)$ that is $(\alpha,\phi)$-linked in $G$, by \emph{starting an CD-process on $U$} we mean that we start a \cp process applied to $G$ and $U$ to deal with, from this timepoint, all the next up to $\lfloor\frac{\phi\vol_{G}(U)}{12}\rfloor$ updates on $G$ that is relevant to $U$ (i.e., an edge insertion/deletion with at least one endpoints of the edge in $U$). %Recall that the CP-process maintains a subset $P\subseteq U$, and we say that the vertices in $P$ are \emph{pruned out} from $U$ by the CP-process.


\subsection{Proof of Lemma~\ref{lem:fully_dynamic_expander_decomposition}}
\label{sec:dyn decomp proof}
%\subsubsection*{The Algorithm for Lemma~\ref{lem:fully_dynamic_expander_decomposition}}


%Throughout the algorithm, we maintain an $(\alpha/38^{\tL}, \phi/38^{\tL})$-partition $\uset$ of vertices of $G$, that is initialized to be the $(\alpha,\phi)$-decomposition of the initial graph $G$.
%and, for each cluster $U\in \uset$, a $U$-counter whose value is either a non-negative integer or a default symbol $\perp$. For a cluster $U\subseteq V$, 
%By \emph{initializing $U$ into $\cal{U}$}, we mean adding the cluster $U$ into $\cal{U}$ and starting an CD-process on $U$ in $G$.
%We now start describing the algorithm.
%\iffalse
%We consider the following cases upon an update on $G$.
%\paragraph{Case 1. Vertex insertion.} 
%If the update is a vertex insertion, we simply create a new cluster in $\uset$ that contains only this new vertex.
%\paragraph{Case 2. Intra-cluster edge insertion/deletion.} 
%If the update is an edge insertion/deletion within a cluster $U$, then we feed an update to the CD-process of $U$ in $G$, which is the insertion/deletion of the corresponding edge, and obtain a subset $Q\subseteq U$ of vertices that are newly pruned out after this update. 
%\iffalse
%We then compute an $(\alpha,\phi)$-decomposition of $Q$ in $G$ and let $Q_1,\ldots,Q_{r'}$ be the clusters we get. We replace the cluster $U$ by the cluster $U\setminus Q$ and decrease the $U$-counter by $1$, and then continue the EP-process on it. For each $1\le j\le r'$, we initialize the cluster $Q_j$ into $\cal{U}$.
%\fi
%\paragraph{Case 3. Inter-cluster edge insertion/deletion.} If the update is an edge insertion/deletion of an edge that connects vertices from two distinct clusters of $\cal{U}$: $v$ from $U$ and $v'$ from $U'$, we feed the deletion of a self-loop on $v$ to the CD-process of $U$ in $G$, and we feed the deletion of a self-loop on $v'$ to the CD-process of $U'$ in $G$.
%\fi
%Let $Q$ ($Q'$, resp.) be the set newly pruned out from $U$ ($U'$, resp.) after this update. We compute an $(\alpha,\phi)$-decomposition of $Q\cup Q'$ in $G$ and let $Q_1,\ldots,Q_{r'}$ be the clusters we get. We replace the clusters $U$ and $U'$ by the clusters $U\setminus Q$ and cluster $U'\setminus Q'$, and continue the EP-process on it. We set the counter of the cluster $U\setminus Q$ ($U'\setminus Q'$, resp.) to be the counter of $U$ ($U'$, resp.) before the update minus $1$. For each $1\le j\le r'$, we initialize the cluster $Q_j$ into $\cal{U}$.
%Whenever the counter of some cluster $U$ expired after an update, we terminate all the CD-process on its sub-clusters, and compute an $(\alpha,\phi)$-decomposition on $U$ in the current graph and start a new CD-process on each cluster in the obtained decomposition. We call this a \emph{recycle operation}. 
%Let $W_1,\ldots,W_{r'}$ be the clusters we get. We delete from $\cal{U}$ the clusters whose counter is $0$ and terminate their EP-process. For each $1\le j\le r'$, we initialize the cluster $W_j$ into $\cal{U}$.
%\iffalse
%We first show (i). See Figure~\ref{fig:boundary_edge} for an example of Case 3. First, from Lemma~\ref{lem:dynamic_expander_pruning}, $|E_{G}(Q,U\setminus Q)|=O(1)$. Since $U$ is $\frac{1}{\log^5m}$-boundary linked, the number of edges in $E_G(Q,V(G)\setminus U)$ is at most $\log^5n$. Note that the clusters $Q_1,\ldots,Q_t$ are obtained from an $(\frac{1}{\log^5m},\phi)$-expander decomposition of $G\{Q\}$. From Lemma~\ref{lem:dynamic_expander_pruning}, $\vol_{G}(Q)=O(1/\phi)$. From Theorem~\ref{thm:strong_expander_decomposition}, the number of edges between clusters $Q_1,\ldots,Q_t$ is at most $\phi\log^5m\cdot O(1/\phi)=O(\log^5m)$. This completes the proof of (i).
%\begin{figure}[h]\centering
%	\includegraphics[scale=0.5]{boundary_edge.jpg}
%	\caption{The partition of cluster $U$ into cluster $U\setminus Q$ and clusters $Q_1,\ldots,Q_t$; the new edges of $E_{G}(Q,U\setminus Q)$ are shown in red; and the new edges between clusters $Q_1,\ldots,Q_t$ are shown in green.}
%	\label{fig:boundary_edge}
%\end{figure}
%\fi

%For each update, if it is in Case 1, then it is clear that the update time is $O(1)$. If it is either in Case 2 or 3, then the update time can be divided into three parts: the time for the existing EP-process, the time for computing an $(\alpha,\phi)$-decomposition in the pruned-out part, and the time for recycle operation. From Lemma~\ref{lem:advanced_dynamic_expander_pruning}, the amortized update time in the EP-process is $\tilde{O}(\psi\cdot(38^\tL/\phi)^2)$, and the volume of the subsets that are newly pruned out is $O(38^\tL/\phi)$. From Theorem~\ref{thm:strong_expander_decomposition}, the update time for computing an $(\alpha,\phi)$-decomposition on the cluster consisting of vertices that we newly pruned out is $\tilde O(38^\tL)$. For the time of recycle. we define a charging scheme to bound it.

%It remains to bound the number new boundary edges. For each update, if it is in Case 1, then it is clear that the number of new boundary edges is $O(1)$. If it is either in Case 2 or 3, then the new boundary edges can be divided into three parts: the new boundary edges from the existing EP-process, the new boundary edges from computing an $(\alpha,\phi)$-decomposition in the pruned-out part, and the new boundary edges for recycle operation. From Lemma~\ref{lem:advanced_dynamic_expander_pruning}, the amortized number of new boundary edges from the existing prune process is $O(\psi)$. {\color{red}to expand} We can deduce that the amortized number if new boundary edges from the the expander decomposition on the newly pruned out part is $O(\psi)$. For the new boundary edges from the recycle operation. we define a charging scheme to bound it. From Theorem~\ref{thm:strong_expander_decomposition}, whenever some $(\alpha,\phi)$-decomposition is performed on some cluster $V'$, it is because there is a set of clusters $U_1,\ldots,U_{r'}$, such that $V'=\bigcup_{1\le j\le r'}U_j$, and for each $1\le j\le r'$, the cluster $U_j$ has endure $\lfloor\frac{\phi\vol_{G}(U_j)}{12}\rfloor$ updates in its EP-process. Therefore, let $m'=\sum_{j=1}^{r'}\vol_{G}(U_j)$, then the total number of updates that the clusters $U_1,\ldots,U_r$ have endured is $\Omega(\phi m')$. On the other hand, the new boundary edges for recycle $V'$ is $\tilde{O}(\phi m)$. We charge the running time of the $(\alpha,\phi)$-decomposition uniformly to the updates endured by the clusters clusters $U_1,\ldots,U_{r'}$. So each update is charged $\tilde{O}(1)$. Therefore, the amortized update time for the recycle operation is $\tilde{O}(1)$. From the above discussion, the amortized number of new boundary edges for our algorithm is $\tilde{O}(\psi)$.
%\fi
We now describe the algorithm for Lemma~\ref{lem:fully_dynamic_expander_decomposition}. %which is extremely simple once we have the CD-process.
First we compute an $(\alpha,\phi)$-decomposition of $G$ using Theorem~\ref{thm:decomp} as a pre-processing step. 
For each cluster $U_i$ in the decomposition for which Theorem~\ref{thm:decomp} returns $\phi_i \ge \phi$ and guarantees that $U_i$ is $(\alpha,\phi')$-linked in $G$, 
we start a CD-process on $U_i$ with the parameters $\alpha,\phi_i$. This completes the description of the algorithm for Lemma~\ref{lem:fully_dynamic_expander_decomposition}.

\paragraph{Bounding the Number of Inter-cluster Edges}\thatchaphol{is this ok?}
From the \cp and the \mlp, it is clear that each cluster $U_i$ in the partition maintained by the algorithm is $(\alpha/38^{L}, \phi/38^{L})$-linked in $G$ because $\phi_i \ge \phi$.
We first show that the the number of inter-cluster edges between the clusters in the partition maintained is bounded by $\tilde O(\phi \vol(G))$.
From Theorem~\ref{thm:decomp}, after pre-processing, the number of inter-cluster edges in the initial partition is $\tilde O(\phi \vol(G))$.
Since the total number of updates is $O(\phi \vol(G)/(\psi\cdot 38^L/\alpha))$, if we can show that the amortized recourse for the contracted graph is $\tilde O(\psi\cdot 38^L/\alpha)$, then at the end of the sequence of updates, the number of edges in the contracted graph is at most 
$\tilde O(\phi \vol(G))+\tilde O(\psi\cdot 38^L/\alpha)\cdot O(\phi \vol(G)/(\psi\cdot 38^L/\alpha))=\tilde O(\phi \vol(G))$.
Therefore, it remains to bound the amortized update time and amortized recourse between the contracted graphs before and after an update.

\paragraph{Amortized update time.}
%We now proceed to bound the amortized update time due to recycling.
From the definition of \cp process, whenever some cluster $U$ expires, it is because its CD-process has handled $\lfloor\frac{\phi'\vol_{G'}(U)}{12}\rfloor$ updates in its previous \cp process, where $G'$ is the graph when the \cp process on $U$ was started, and $\phi'$ is the expansion parameter of $U$ when the CD-process on it was started. 
Observe that the current volume of $U$ in the current graph $G$ is at most $\vol_{G'}(U)+O(\phi'\vol_{G'}(U))=O(\vol_{G'}(U))$.
Moreover, since initially the number of boundary edges of $U$ is at most $\tilde O(\phi'\vol_{G'}(U))$ (from the definition of an $(\alpha,\phi')$-decomposition), and the number of updates that the CD-process on $U$ has handled is $\tilde O(\phi'\vol_{G'}(U))$, it can be derived that, when $U$ is being recycled, the number of its boundary edges is at most $\tilde O(\phi'\vol_{G'}(U))$.
Therefore, from Theorem~\ref{thm:decomp}, the time for recycling $U$ is $\tilde{O}(\vol_{G'}(U)/\phi')$.
We charge this uniformly to the updates handled by its CD-process. 
Therefore, the amortized update time for the recycling is $\tilde{O}(1/\phi'^2)=\tilde{O}(1/\phi^2)$.
Note that, from the algorithm, the cluster $U$ and the parameter $\phi'$ that is given to the CD-process is always a cluster of some $(\alpha,\phi)$-expander decomposition produced by the algorithm in Theorem~\ref{thm:decomp}. Therefore, $\phi'\ge \phi$ always holds, and the amortized update time for the recycling is $\tilde{O}(1/\phi'^2)=\tilde{O}(1/\phi^2)$.
Combined with previous discussion on the amortized update time of a CD-process, the amortized update time for the algorithm is $\tilde{O}(\frac{\psi\cdot 38^{2L}}{\alpha\phi^2})$.
%From the above discussion, the amortized update time for our algorithm is $\tilde{O}(\psi\cdot(38^L/\phi)^2)$.

\paragraph{Amortized recourse.}
Let $U$ be a cluster that is $(\alpha,\phi')$-linked in $G$ when the CD-process on it is started. 
We consider the amortized recourse in cluster $U$. 
The recourse between the contracted graphs before and after an update can be divided into two parts, the recourse inside $U$ and the recourse between $U$ and $V\setminus U$ (or equivalently, the recourse within the edges of $\Gamma_G(U)$). 

We first consider the case where $U$ does not expire after an update.
Recall that the CD-process maintains the sets $\tilde P^1,\ldots,\tilde P^{\tL}$.
Assume first that the sets $\tilde P^2,\ldots,\tilde P^{\tL}$ do not change after this update, then only the clusters $\tilde P^1$ and $U\setminus \tilde P^1$ change. 
Note that, from Theorem~\ref{thm:dynamic_expander_pruning}, $\vol(\tilde P^1)\le O(\psi\cdot 38^{\tL}/\phi')$, and from Observation~\ref{obs:downward_inter}, $|E(\tilde P^1, V\setminus \tilde P^1)|\le O(\psi/\alpha)$.
Therefore, after computing an $(\alpha,\phi')$-decomposition on $\tilde P^1_i$ using Theorem~\ref{thm:decomp}, the number of the inter-cluster edges between these clusters is $O(\psi\cdot 38^{\tL}/\alpha)$,
%Moreover, from Observation~\ref{obs:intra}, $|E(\tilde P^1,U\setminus \tilde P^1)|=O(\psi)$ always holds. 
and the amortized recourse is at most $O(\psi\cdot 38^{\tL}/\alpha)$.
Assume now that the set $\tilde P^s$ changes for some $2\le s\le \tL$. Recall that this happens after every $\psi^{s}$ updates on $\tilde P^s$.
%According to \cp, the sets $\tilde P^1,\ldots,\tilde P^{s-1}$ change as well, and we recompute an $(\alpha,\phi')$-decomposition individually on each of the clusters $\tilde P^1,\ldots,\tilde P^s$.
From the Observation~\ref{obs:intra} and~\ref{obs:downward_inter}, the number of new inter-cluster edges between clusters in $\tilde P^s$ is $\tilde O(\psi^s\cdot 38^{\tL}/\alpha)$. 
Therefore the amortized recourse is $\tilde O(38^{\tL}/\alpha)$.
%We charge this uniformly to the $\psi^{s}$ updates handled by machine $M_s$ in this stage, so each update is charged $\tilde O(\psi\cdot 38^{\tL}/\alpha)$. 
Summing over all $1\le s\le \tL$, we get that the amortized recourse in cluster $U$ is $\tilde O(\psi\cdot 38^{L}/\alpha)$.


For the recourse between $U$ and $V\setminus U$. We first consider the recourse in $E(\tilde P^s,V\setminus U)$ for each $1\le s\le \tL$ separately. Fix an index $2\le s\le \tL$. From Observation~\ref{obs:downward_inter}, the number of edges in $E(\tilde P^s,V\setminus U)$ is always at most $O(\psi^s/\alpha)$. Since the set $\tilde P^s$ and the subpartition on $\tilde P^s$ maintained by the CD-process on $U$ change every $\psi^s$ updates, the amortized recourse in $E(\tilde P^s,V\setminus U)$ is $O(1/\alpha)$.
Now consider the recourse in $E(\tilde P^1,V\setminus U)$. Again from Observation~\ref{obs:downward_inter}, the number of edges in $E(\tilde P^s,V\setminus U)$ is always at most $O(\psi/\alpha)$. Therefore, the amortized recourse in $E(\tilde P^s,V\setminus U)$ is also bounded by $O(\psi/\alpha)$. Altogether, the amortized recourse in $E(P^1,V\setminus U)$ is $O(\psi/\alpha)$.
On the other hand, the recourse in $E(U\setminus P^1,V\setminus U)$ can be also divided into two parts: (i) an edge in $E(U\setminus P^1,V\setminus U)$ is inserted or deleted; or (ii) an edge in $E(U\setminus P^1,V\setminus U)$ is moved to 
$E(P^1,V\setminus U)$ due to the change on the partition maintained by the CD-process.
The amortized recourse for updates in (i) is clearly $O(1)$. Observe that each recourse in (ii) corresponds to one recourse in $E(P^1,V\setminus U)$. Therefore, the amortized recourse in (ii) is $O(\psi/\alpha)$.
Altogether, the amortized recourse between $U$ and $V\setminus U$ is $O(\psi/\alpha)$.

\iffalse
For the recourse between between $U$ and $V\setminus U$, we use the following observation, that follows immediately from Observation~\ref{obs:cluster_linkedness}.
\begin{observation}
For each $1\le s\le \tL$, $|E(\tilde{P}^s,V\setminus U)|\le O\left(|E\left( \tilde{P}^s,U\setminus(\bigcup_{s\le j\le \tL}\tilde P^j) \right)|/(\alpha/38^{\tL-s})\right)$.
\end{observation}
Since the amortized recourse inside the cluster $U$ is $O(\psi\cdot 38^{\tL}/\alpha)$, from the above observation, the recourse in $\Gamma_G(U)$ caused by $\tilde P^s$ is at most $O(\psi\cdot 38^{2L}/\alpha^2)$ for each $s$\thatchaphol{why?}. Summing up over all $1\le s\le \tL$, the amortized recourse within $\out(U)$ is $\tilde O(\psi\cdot 38^{2L}/\alpha^2)$.
\fi

We consider next the recourse caused by the recycling. Let $U$ be a cluster that expires after the current update. 
We first consider the amortized recourse inside $U$.
Assume that $U$ was $(\alpha,\phi')$-linked when the CD-process on it was started.
Therefore, from Theorem~\ref{thm:decomp}, at that time the number of edges between $U$ and $V\setminus U$ is at most $\phi'\vol(U)$. Since $U$ has handled $O(\phi'\vol(U))$ updates before it expires, at the time when it expires, the number of edges edges between $U$ and $V\setminus U$ is $O(\phi'\vol(U))$.
From the algorithm, we recompute an $(\alpha,\phi)$-decomposition on $U$ in the current graph. From Theorem~\ref{thm:decomp}, the total number of edges between these clusters is at most 
$\tilde O\left(\phi'\vol(U)+\phi\vol(U)\right)=\tilde O\left(\phi'\vol(U)\right)$.
We charge this uniformly to all updates that its CD-process has handled, then the amortized recourse is $\tilde{O}(1)$.  
We now consider the amortized recourse in $E(U,V\setminus U)$.
From Theorem~\ref{thm:decomp}, after we recompute the $(\alpha,\phi)$-decomposition on $U$, the number of edges between $U$ and $U\setminus V$ is 
%\zihan{add reference here}
$\tilde O\left(\phi'\vol(U)\right)$.
Therefore, the amortized recourse is $\tilde{O}(1)$. 

Altogether, the amortized recourse for the algorithm is $\tilde O(\psi\cdot 38^{L}/\alpha)$.
 


























==> dynamic_expander_hierarchy.tex <==
\section{Fully Dynamic Expander Hierarchy}
\label{sec:proof_of_fully_dynamic_expander_decomposition}

In this section, we will show an algorithm that maintains an expander hierarchy of an unweighted simple graph that undergoes edge insertions and deletions. To maintain the expander hierarchy, we will construct auxiliary unweighted multi-graphs with self-loops. The dynamic graph $G$ that we will be dealing with has $n$ vertices, and we let $m$ to be an upper bound of the number of edges in $G$ at any time. Since $G$ is an unweighted simple graph at any time, we have $m=O(n^2)$ and $\log m=O(\log n)$. Our main result in this section is the following theorem.

\begin{theorem}
\label{thm:dynamic_R_tree}
There is a randomized algorithm that, given any unweighted graph $G$ on $n$ vertices undergoing adaptive edge insertions and deletions, maintains, with high probability, a $2^{-O(\sqrt{\log n})}=n^{-o(1)}$-expander hierarchy of $G$ in worst-case update time $2^{O(\log^{3/4} n)}=n^{o(1)}$.
\end{theorem}

In Section~\ref{subsec:warmup}, we introduce some new notations and subroutines, and then provide a proof of a weaker bound to familiarize the use of them and to illustrate the main ideas of maintaining the expander hierarchy via maintaining the boundary-linked expander decomposition of the graph on each level.

In Section~\ref{subsec:decremental}, we provide a proof of the \emph{amortized} version of Theorem~\ref{thm:dynamic_R_tree}, namely we can maintain a $2^{-O(\sqrt{\log n})}$-EH of $G$ in amortized time $2^{O(\sqrt{\log n})}$, such that in every phase, a property called the \emph{decremental expander property} is satisfied. This property is crucial for the application of maintaining dynamic low-stretch spanning forest in Section~\ref{sec:application_dynamic}.

Last, we will provide in Section~\ref{subsec:fully_dynamic_expander_decomposition} an alternative proof of the amortized version of Theorem~\ref{thm:dynamic_R_tree}, showing that a $2^{-O(\sqrt{\log n})}$-EH of $G$ can be maintained in \emph{amortized} time $2^{O(\log^{3/4} n)}$, and then we show how to de-amortize it and finally obtain the proof of Theorem~\ref{thm:dynamic_R_tree}.

==> dynamic_expander_hierarchy_decremental.tex <==
\subsection{$n^{o(1)}$ Amortized Time Decremental Expander}
\label{subsec:decremental}

In this section we construct an algorithm that maintains a $\phi$-EH in amortized time $2^{O(\sqrt{\log n})}$. We fix $\phi=2^{-\Theta(\sqrt{\log m})}=n^{-o(1)}$. We will use the notations in the proof of Lemma~\ref{lem:warm_up_dynamic_expander_decomposition}.

Similar to the last section, we still first divide the updates of $G$ into phases, but now we let each phase consist of $\phi m/12$ consecutive updates. At the beginning of each phase, we recompute a $\phi$-EH of $G$ using Lemma~\ref{lem:static_EH_construction}.
Let $t$ be the depth of the $\phi$-EH.
In each phase, we maintain a \phiep{ }for every graph $G^{i}$.
Specifically, for each $0\le i\le t$, we denote by $\uset^i$ the partition of $V(G^i)$ that we maintain. For each $0\le i\le t$, denote $\uset^i=\{U^i_1,\ldots,U^i_{\ell_i}\}$, where $\ell_i=|\uset^i|$. 
For each cluster in $\uset^i$ for some $i$, we additionally maintain a counter that always contains an integer or a default symbol $\perp$.
For each $0\le i\le t$ and each $1\le j\le \ell_i
$, we initialize the cluster $U^i_j$ into $\uset^i$.



We consider the following cases upon an update of $G$.

\textbf{Case 1.} 
If the update is a vertex insertion, then for each $G^i$, we add this vertex into $G^i$, create a new cluster that only contains this new vertex, and initialize this cluster into $\uset^i$.

\iffalse
If the update is an edge insertion/deletion of $(v,v')$ such that the $v$ and $v'$ belong to different clusters in $\uset^0,\ldots,\uset^i$, but belong to the same cluster of $\uset^{i+1}$, then we do the following.
\fi

\textbf{Case 2.} 
If the update is an edge insertion/deletion of an edge within a cluster of $\uset^0$, then we feed an update to the EP-process of $G\{U\}$, which is the insertion/deletion of the corresponding edge, and obtain a subset $Q\subseteq U$ of vertices that are newly pruned out after this update. 
We replace the cluster $U$ by the cluster $U\setminus Q$ while setting the counter of the cluster $U\setminus Q$ to be the counter of $U$ before the update minus $1$, and then continue the EP-process on it.
Now, for the set $Q$, we no longer perform a \phied\text{ }on it. Instead, for each vertex in $Q$, we create a new cluster that contains only this new vertex, and initialize this cluster into $\uset^0$. 

\textbf{Case 3.}
If the update is an edge insertion/deletion that connect vertices from two distinct clusters of $\uset^0$: $v$ from $U$ and $v$ from $U'$, we feed an update to the EP-process of $G\{U\}$, which is the deletion of an self-loop on vertex $v$, and we feed an update to the EP-process of $G\{U'\}$, which is the deletion of an self-loop on vertex $v'$. Let $Q$ ($Q'$, resp.) be the set newly pruned out from $U$ ($U'$, resp.) after this update.
We replace the cluster $U$ by the cluster $U\setminus Q$ while setting the counter of the cluster $U\setminus Q$ to be the counter of $U$ before the update minus $1$, and then continue the EP-process on it.
Now for each vertex in $Q\cup Q'$, similar to the previous case, we create a new cluster that only contains this new vertex, and initialize this cluster into $\uset^0$. 

Now let $\uset^0_s\subseteq \uset^0$ be the collection of newly-added singleton clusters (each contains a single vertex from $Q\cup Q'$). We will explain how to maintain the partitions $\uset^1\ldots,\uset^t$. Once the partitions $\uset^1\ldots,\uset^t$ are properly maintained, for each $0\le i\le t$, the graph $G^i$ is simply maintained as the contracted graph of $G^{i-1}$ with respect to the partition $\uset^i$, namely $G^i=G^{i-1}_{\uset^i}$. 

We begin with updating $G^1$ and $\uset^1$ based on $\uset^0_s$.
Note that, by our way of maintaining $\uset^0$, all singleton clusters in $\uset^0$ are added into the graph $G^1$, and all the edges incident to them in $G^0$ are copied into $G^1$ as well. Note that, the node $u$ in $G^1$ representing the cluster $U$ of $G^0$ in Case 2, or the nodes $u',u''$ in $G^1$ representing the clusters $U'$ and $U''$ of $G^0$ respectively in Case 3, may have incident edges to the singleton clusters in $\uset^0$.
From the viewpoint of $G^1$, this may cause self-loops to be added to or deleted from the cluster of $\uset^1$ that contains the node $u$ or the nodes $u'$ and $u''$. We feed updates accordingly to the EP-process of the corresponding cluster(s) in $\uset^1$, which is the insertion/deletion of $O(1)$ self-loops on $u$ (in Case 2) or on $u'$ and $u''$ (in Case 3). Let $Q^1$ be the set of vertices that is newly pruned out. We initialize each node of $Q^1$ into $\uset^1$, and let $\uset^1_s$ be the union of $\uset^0_s$ and all singleton clusters of vertices of $Q^1$. Then we proceed to update $G^2$ and $\uset^2$ based on $U^1_s$ in the same way, and so on, up to $G^t$ and $\uset^t$.

For each $1\le i\le t$, we also set a \emph{volume threshold} on the graph $G^i$ that is defined as follows. It is clear that, at the beginning of each phase, after we recompute the whole EH, the volume of each $G_i$ is at most $(C\phi\log^5m)^im$ for some constant $C$. We set the volume threshold of graph $G^i$ to be $\vt_i=2(C\phi\log^5m)^im$. %\gramoz{The pruning algorithm can support only up to $\phi |E(G^{i})|$ updates at level $i$ and we have not discussed the possible rebuilds that might occur before the volume threshold is reached}
Whenever the volume of some $G^i$ reaches $\vt_i$, we recompute the sub-EH from the $i$th level up to the top level. That is, we compute a $\phi$-EH of $G^i$ using Lemma~\ref{lem:static_EH_construction}, and replace the sub-tree until the level of $G^i$ of the original EH by the new one.

Whenever for some $G^i$, the counter of some cluster in $\uset^i$ becomes $-1$ after an update, we let $\tilde{U}$ be the union of such clusters, and recompute a \phied\text{ }on $G\{\tilde{U}\}$. Let $W_1,\ldots,W_{r'}$ be the clusters we get. We delete from $\uset^i$ the clusters whose counter is $-1$ and terminate their EP-process. For each $1\le j\le r'$, we initialize the cluster $W_j$ into $\uset^i$. We update the partitions $\uset^{i+1},\ldots,\uset^{t}$ accordingly.

The \emph{decremental expander property} is that, in each phase, for each $0\le i\le t$, between two recomputation of the sub-EH from the level of $G^i$ above, the partition $\uset^i$ only becomes \emph{finer}, in the sense that, whenever two vertices are in distinct clusters of $\uset^i$, they will no longer belong to the same cluster of $\uset^i$ before the next sub-EH-initialization. From the algorithm, it is clear that the decremental expander property is satisfied.

\iffalse
Similar to the previous section, whenever in some graph $G^i$, the counter of some cluster becomes $-1$ after an update, we let $\tilde{U}$ be the union of such clusters, and recompute a \phied\text{ }on $G^{i}\{\tilde{U}\}$. Let $W_1,\ldots,W_t$ be the clusters we get. We delete from $\cal{U}$ the clusters whose counter is $-1$ and terminate their EP-process. For each $1\le j\le t$, we initialize the cluster $W_j$ into $\cal{U}$, and update $\uset^{i+1},\ldots,\uset^{t}$ according to it.
\fi

It is clear that the above algorithm maintains a valid $\phi$-EH throughout. It remains to analyze the update time. Similar to the proof of Lemma~\ref{lem:warm_up_dynamic_expander_decomposition}, the amortized update time for recomputing the \phied\text{ }can be bounded by $\tilde{O}(1/\phi^2)$. It suffices to bound the amortized update time for recomputing the sub-EH.

For each $0\le i\le t$, we denote by $\hat{U}^i$ to be the set of vertices that form singleton clusters in $\uset^i_s$.
\begin{proposition}
\label{pro:volume}
For each $k$, and for each $1\le i\le t$, after the $k$th update, $\vol_{G_i}(\hat{U}^i)\le 16^{i+1}\cdot k/\phi$.
\end{proposition}
\begin{proof}
We prove by induction on $i$. The base case is where $i=0$. The set of vertices of $\hat{U}^0$ after the $k$th update is the union of all pruned sets among the first $k$ updates. From Lemma~\ref{lem:dynamic_expander_pruning}, the volume of this set is at most $8k/\phi$. Assume the proposition is true for $\hat{U}^0,\hat{U}^1,\ldots,\hat{U}^{i-1}$, now consider the set $\hat{U}^i$. From the algorithm, the set $\hat{U}^i$ can be divided into two subsets: (i) the set $\hat{U}^{i-1}$; and (ii) the newly-pruned set $\tilde{U}^i$ caused by adding the singleton clusters of vertices from set $\hat{U}^{i-1}$. From the induction hypothesis $\vol_{G^{i-1}}(\hat{U}^{i-1})\le 16^{i}\cdot k/\phi$. Therefore, the accumulative number of self-loop insertions and deletions incident to nodes of $G^i$ is at most $2\cdot 16^{i}\cdot k/\phi$. From Lemma~\ref{lem:dynamic_expander_pruning}, $\vol_{G_i}(\hat{U}^{i})\le 16^{i+1}\cdot k/\phi$.
\end{proof}
Therefore, for the graph $G^i$ to have volume above $\vt_i$ so that recomputing the sub-EH from this level above is necessary, we need $k$ updates where $16^{i+1}\cdot k/\phi=(C\phi\log^5m)^im$, which means that the total time that we spent on this level in a phase is 
$\tilde{O}(\phi^{i+1}\log^{O(i)}m\cdot m\cdot (\phi m/k))=\tilde{O}(\phi^{i+1}\log^{O(i)}m\cdot 16^{i}\phi m/(\phi^{i+1}m))=\tilde{O}(16^i\log^{O(i)}m\cdot\phi m)=\phi^{O(1)}m$. By the union bound over all levels from $0$ to $t$, the total update time in recomputing the sub-EH is $\phi^{-O(1)}m$, and therefore the amortized udpate time is $\phi^{-O(1)}=2^{O(\sqrt{\log m})}$.

For the total update time for pruning, from Proposition~\ref{pro:volume}, the total volume of all $\hat{U}^0,\ldots,\hat{U}^t$ is $O(16^t\cdot\phi m/\phi)=\phi^{-O(1)}m$. Therefore, the total update time is $\phi^{-O(1)}m\cdot 1/\phi^2=\phi^{-O(1)}=2^{O(\sqrt{\log m})}$.

Combine the last two paragraphs together, we conclude that the amortized running time is $2^{O(\sqrt{\log m})}$.












==> dynamic_expander_hierarchy_scheduling.tex <==
\subsection{Proof of Theorem~\ref{thm:dynamic_R_tree}}
\label{subsec:fully_dynamic_expander_decomposition}

Fix $\phi=2^{-\Theta(\sqrt{\log m})}=n^{-o(1)}$ and let $t=\log_{1/\phi}m=\Theta(\sqrt{\log m})$.
Fix $\psi=2^{\Theta(\log^{1/4} m)}=n^{o(1)}$ and let $L=\log_{\psi}m=\Theta(\log ^{3/4}m)$.
We will use the following theorem on maintaining a \phied.

\begin{theorem}[Fully Dynamic Expander Decomposition]
\label{thm:fully_dynamic_expander_decomposition}
There is a randomized algorithm, that, given any unweighted graph $G$ on $n$ vertices undergoing a sequence of $k\le \phi m/12$ updates including vertex insertions, edge insertions and deletions, maintains a boundary-linked $(\phi\cdot 6^{-L})$-expander decomposition in worst-case update time $\tilde{O}(\psi\cdot (6^L/\phi)^2)$ and pre-processing time $\tilde{O}(m/\phi)$. Moreover, after each update, the number of new boundary edges is $O(\psi)$.
\end{theorem}

The proof of Theorem~\ref{thm:fully_dynamic_expander_decomposition} is deferred to Appendix~\ref{apd:dynamic_expander_decomposition}. 
We now show the proof of Theorem~\ref{thm:dynamic_R_tree} using Theorem~\ref{thm:fully_dynamic_expander_decomposition}.

First, we show how to maintain the $\phi$-EH with amortized update time $2^{O(\log^{3/4} n)}$ using it. 
The proof is similar to the proof in the previous section. 
We divide the updates of $G$ into phases, such that each phase consist of $\phi m/12(\psi\log n)^t$ consecutive updates. For each phase, we first preprocess the current graph by computing an $\phi$-EH of $G$ using the algorithm in Lemma~\ref{lem:static_EH_construction}, which has depth $t=\Theta(\sqrt{\log m})$. Then upon an update to $G$, we first update $G^0$ accordingly so that $G^0=G$ always hold. Then for each $0\le i\le t-1$, we maintain a \phied \text{ }of $G^{i}$ using the algorithm of Theorem~\ref{thm:fully_dynamic_expander_decomposition}, and set $G^{i+1}$ to be the contracted graph with respect to the \phiep.
Let $t'<t$ be the largest integer such that $(\psi\log n)^{t'}=\Theta(\phi^{t'}m)$, so
so $t'=\Theta(\sqrt{\log m})$ and $\phi^{t'}m=2^{O(\log^{3/4}m)}$.
For the graphs $G^{t'},\ldots,G^t$, upon each update to $G$, we recompute its \phied\text{ }from scratch. 
Note that, from Theorem~\ref{thm:fully_dynamic_expander_decomposition}, an update of $G^i$ may result in at most $O(\psi)$ updates in $G^{i+1}$. Therefore, after $\phi m/12(\psi\log n)^t$ updates to $G$, each graph $G^i$ may encounter at most $\left(\phi m/12(\psi\log n)^t\right)\cdot (O(\psi)^{t})\le \phi m/12$ updates. Therefore, from Theorem~\ref{thm:fully_dynamic_expander_decomposition}, at any time of any phase, for each $1\le i\le t$ the boundary-linked $\phi\cdot 6^{-L}$ expander decomposition of $G^i$ that we maintain is valid.
For the update time, upon each update, it takes $2^{O(\log^{3/4}m)}$ time to recompute the its \phied\text{ }of the graphs $G^{t'},\ldots,G^t$ from scratch, and from Theorem~\ref{thm:fully_dynamic_expander_decomposition}, it takes $\psi^{t'}\cdot(6^L/\phi)^2=2^{O(\log^{3/4}m)}$ time for maintaining the graphs $G^0,\ldots,G^{t'-1}$. 
At the beginning of each phase, from Lemma~\ref{lem:static_EH_construction}, the time needed to recompute the whole expander hierarchy is $\tilde{O}(m/\phi)$.
We charge it uniformly to all the updates in the phase, so each update is charged at most $(\psi\log n)^{t}/\phi^2=2^{O(\log^{1/2}m)}$. Therefore, the amortized update time for maintaining the $\phi$-EH is $2^{O(\log^{3/4}m)}$.

We now show how to maintain the $\phi$-EH with worst-case update time $2^{O(\log^{3/4} n)}$. Note that, in our algorithm, the only part whose running time needs to be amortized is the recomputing the whole expander hierarchy, which happens at the beginning of each phase. Observe that, the reason that we need to recompute an EH from scratch is that the previous EH, which was recomputed at the beginning of the last phase, cannot endure too many updates from Theorem~\ref{thm:fully_dynamic_expander_decomposition}. Therefore, when the number of updates to an newly-computed EH reaches a threshold, which is the number of the updates in a phase, we have to recompute the whole EH \emph{right away} to withstand the new updates. This takes $\tilde{O}(m/\phi)$ time, and according to our algorithm above, this is done in the period of one single update.

The idea to avoid this ``EH-recomputing in one update'' issue is to intuitively distribute the work of an EH-recomputing among the period of a batch of udpates. Specifically, we define the \emph{EH-phases} as follows.
Let $T=\phi m/12(\psi\log n)^t/3$. For each $j$, we start an EH-phase from the $(jT+1)$th update, let it run for $3T$ updates and terminate it at the $(j+3)T$th update. So there are at most $3$ EH-phases running at the same time.
In each EH-phase, we recompute EH of a graph (which will be specified later) from scratch and then maintain it over certain batch of updates.
Among the three EHs that are maintained by different EH-phases, one of them will be designated as the \emph{main EH}, which is the output of the algorithm. Namely, whenever there is a query on the EH that is maintained by the algorithm, the algorithm uses the main EH that it is currently maintaining.

Each EH-phase is divided into three stages, each containing a batch of $T$ consecutive updates. The first and the second stage is called the preparation stage, and the third stage is called the execution stage, in which the EH is finally ``put to work'', in the sense that the expander hierarchy that is maintained in this stage of this EH-phase is designated to be the main EH of the algorithm.
See Figure~\ref{fig:EH_scheduling} for an illustration.

\begin{figure}[h]
\centering
\includegraphics[scale=0.60]{EH_scheduling}
\caption{The scheduling of consecutive EH-phases. The green arrow represents the stages of the main EH. $D(i,j)$ represents the batch of updates from the $i$th to the $j$th.}
\label{fig:EH_scheduling}
\end{figure}

To be specific, we now describe three stages of an EH-phase, which we call the current EH-phase, and its relation to its previous EH-phase.
Let $G$ be the graph at the beginning of the previous EH-phase, and let $G_{T}, G_{2T}, G_{3T}$ and $G_{4T}$ be the graphs after $T,2T, 3T$ and $4T$ updates, respectively.
The current EH-phase starts from the $(T+1)$th update, and ends at the $4T$th update.
In the first stage of the current EH-phase (from the $(T+1)$th update to the $2T$th update), it recomputes an EH of $G_T$, such that after each update in this stage, the running time is $O((\psi\log n)^t/\phi^2)=2^{O(\sqrt{\log n})}$. In the second stage of the current phase, (from the $(2T+1)$th update to the $3T$th update), it sequentially handles the updates from the $(T+1)$th to the $3T$th on the EH that it just computed, by handling two updates after each new update comes. Specifically, it first handles the $(T+1)$th and the $(T+2)$th after the $(2T+1)$th update comes, and then handles the $(T+3)$th and the $(T+4)$th after the $(2T+2)$th update comes, and so on. At the end of this stage, it ``catches up'' all the updates. It is easy to see that in this stage, the running time of after each update is $2^{O(\log^{3/4}m)}$. In the third stage, (from the $(3T+1)$th update to the $4T$th update), the EH is designated as the main EH of the algorithm and it normally handles all updates, which takes time $2^{O(\log^{3/4}m)}$ per update. Note that, from Theorem~\ref{thm:fully_dynamic_expander_decomposition}, each EH that is maintained in an EH-phase, after it is initially computed from scratch, can endure $3T$ updates. Therefore, at any time, the EH that we maintain in this way is valid, and in this way we manage to get $2^{O(\log^{3/4}m)}$ worst-case update time.











